DARKSIDE: A Heterogeneous RISC-V Compute Cluster for Extreme-Edge On-Chip DNN Inference and Training

On-chip DNN inference and training at the Extreme-Edge (TinyML) impose strict latency, throughput, accuracy and flexibility requirements. Heterogeneous clusters are promising solutions to meet the challenge, combining the flexibility of DSP-enhanced cores with the performance and energy boost of dedicated accelerators. We present DARKSIDE, a System-on-Chip with a heterogeneous cluster of 8 RISC-V cores enhanced with 2-b to 32-b mixed-precision integer arithmetic. To boost performance and efficiency on key compute-intensive Deep Neural Network (DNN) kernels, the cluster is enriched with three digital accelerators: a specialized engine for low-data-reuse depthwise convolution kernels (up to 30 MAC/cycle); a minimal overhead datamover to marshal 1-b to 32-b data on-the-fly; a 16-b floating point Tensor Product Engine (TPE) for tiled matrix-multiplication acceleration. DARKSIDE is implemented in 65nm CMOS technology. The cluster achieves a peak integer performance of 65 GOPS and a peak efficiency of 835 GOPS/W when working on 2-b integer DNN kernels. When targeting floating-point tensor operations, the TPE provides up to 18.2 GFLOPS of performance or 300 GFLOPS/W of efficiency - enough to enable on-chip floating-point training at competitive speed coupled with ultra-low power quantized inference.

==> 01_Introduction.tex <==
\section{Introduction}
% Intro of the problem
The number of AI-enhanced IoT applications is growing fast~\cite{niculescu2021improving, sun2019ai}, calling for a new class of microcontroller devices capable of sustaining intense Machine Learning (ML) and Deep Learning (DL) workloads, in addition to more traditional tasks for IoT end-nodes, such as data acquisition and transmission. All within a power envelope of few tens of milliWatts and without sacrificing the programmability.

% TinyML requirements
ML and DL algorithms deployed at the extreme-edge of IoT, usually referred to as TinyML~\cite{ray2021review}, require advanced capabilities, including not only on-chip inference tasks performed by employing low-cost reduced integer arithmetic, but also DNN model tuning, partial on-chip training~\cite{ravaglia2021tinyml} or unsupervised continual learning tasks~\cite{unknown}, which are instead performed with more costly floating-point data representation. 

% Heterogeneous Computing
Heterogeneous compute fabrics are a promising solution to deliver TinyML's required performance, efficiency and flexibility while coping with strict power and cost constraints~\cite{VEGA}: multiple programmable cores provide flexible and efficient execution for generic parallel kernels, while specialized hardware accelerators provide extra performance and efficiency boost on key kernels that dominate the computational workload.

% Inference 
For inference tasks on extreme-edge devices, a common direction of TinyML is to shrink the models through quantization-aware~\cite{jacob2018quantization} and post-training quantization techniques~\cite{hubara2017quantized}, adopting low-bitwidth integer arithmetic. In this domain, the mixed-precision approach~\cite{rusci2020leveraging}, where the activations and the weights of the DNN are quantized asymmetrically, has demonstrated its efficacy to fit the limited memory resources of microcontroller systems, while reducing the Top-1 accuracy drop gap, compared to the full-precision floating point model, within a 3 to 6\% range, which is acceptable for AI-enhanced IoT applications. 

% MIXED -- ASIC
Hence, low- and mixed-precision DNNs are one of the critical kernels to accelerate in extreme-edge devices. Low-precision arithmetic is widely adopted into state-of-the-art specialized digital data-paths~\cite{chen2019eyeriss, moons201714, lee2018unpu, desoli201714} or in analog-digital mixed-signal solutions~\cite{khaddam2022hermes, ueyoshi2022diana} to boost the energy efficiency of DNN inference tasks, in the orders of ten to hundreds TOPS/W. However, these hardware blocks lack flexibility to map different workloads than the ones for which they are designed for and must be coupled with processors to be usable in the IoT world, with increased area and power costs.

% MIXED -- ISA
An alternative approach, which improves the computation efficiency without additional area costs and without compromising the programmability, is to introduce hardware-accelerated extensions for low-precision integer arithmetic within the ISA of general-purpose processors. Authors of~\cite{garofalo2021xpulpnn} propose RISC-V SIMD sum-of-dot-product instructions and custom mac-load operations to achieve ASIC-like efficiency on symmetric DNN convolutions. Other works~\cite{ottavi2020mixed} move forward implementing light-weight status-based mixed-precision computing support to a RISC-V processor, showing two orders of magnitude better efficiency than existing commercial microcontroller solutions.

% DEPTHWISE and DATA MARSHALING
However, there exist some kernels which are intrinsically challenging to parallelize with the previously mentioned techniques. Depth-wise convolution layers have less computation complexity and less footprint compared to standard convolutions, but they are not computationally efficient, due to their poor intrinsic data reuse \cite{garofalo2022heterogeneous}. In the DNN processing pipeline, the Amdahl's effect moves soon toward depth-wise kernels which become the computing bottleneck, demanding new solutions for depth-wise kernels acceleration, addressed in this work. Likewise, data marshaling operations (e.g., low-bitwidth transpose) commonly used in DNNs are inefficient as they heavily rely on sub-byte swap operations.

% What about training
Other kernels require a performance boost that cannot be achieved without using a massive number of cores, which would blow up the SoC's area unacceptably. In particular, on-chip learning requires floating-point (FP) arithmetic, and the workload is 10-100$\times$ larger than inference~\cite{ravaglia2021tinyml}. While recent work has shown that FP16 and even FP8 can be used ~\cite{rodriguez2018lower, sun2019hybrid}, the performance requirements are very high and require fixed-function acceleration to fit within a TinyML compatible area budget.

% Our solution
In this work, we present \textsc{Darkside}, a PULP-based~\cite{starwars, VEGA} heterogeneous computing SoC that targets emerging TinyML inference and on-chip training applications.
We introduce four main innovations in \textsc{Darkside}: \textit{1)} RISC-V cores with advanced low-bitwidth mixed-precision integer computing capabilities; three dedicated hardware accelerators:  \textit{2)} a Depth-Wise convolution Engine (DWE), \textit{3)} a low-overhead DataMover for marshaling operations, and \textit{4)} a low-power Tensor Product Engine (TPE) for efficient FP16 matrix multiplications.
The cores and accelerators are tightly integrated into a shared-L1 cluster to enable advanced hardware/software cooperation. The chip has been fabricated in TSMC 65nm technology and shows peak integer performance (2-bit) of 65 GOPS with an efficiency of 835 GOPS/W. On TPE-accelerated FP16 workloads, it achieves up to 18.2 GFLOPS and a peak efficiency of 300 GFLOPS/W at 2.6 GFLOPS, achieving peak performance and efficiency similar to 8-bit integer operations.


==> 01_v2_Introduction.tex <==
\section{Introduction}
% TinyML requirements -- inference okv0
Recently, the research effort to deploy \ac{ML} and \ac{DL} algorithms at the extreme-edge of the \ac{IoT}, usually referred to as Tiny Machine Learning (\textit{TinyML}), has reached outstanding results, making it possible to deploy complex \ac{DL} models on such tiny systems. As an example, MobileNets~\cite{sandler2018mobilenetv2} have rapidly become the state-of-the-art compute workloads integrated in \ac{IoT} computer vision pipelines. These models can be used both for classification and object detection inference tasks, but also employed as a flexible template for tasks not related to vision~\cite{cai2018proxylessnas,incze2018bird, zhang2019lightweight}. 

% TinyML -- training okv0
Besides, many AI-enhanced \ac{IoT} applications require the deployed \ac{DL} model to adapt to new data and scenarios to keep unaltered the accuracy of the prediction. Re-train a model liike a \ac{DNN} on data-centers collecting on-field data from the distributed \ac{IoT} end-nodes and then re-upload the model on the edge devices might be expensive in terms of latency and power costs. A common direction of TinyML is to rethink the deployed \ac{DNN} as a dynamic model that can improve and adapt itself by learning from new sensed data directly on the end-nodes. Recent progress in this research area concern \ac{DNN} model tuning, partial on-chip training~\cite{ravaglia2021tinyml} or unsupervised continual learning tasks~\cite{ren2021tinyol}, which have been applied successfully to a wide range of \ac{IoT} applications, such as anomaly detection tasks~\cite{unknown}. 

% new generation of IoT devices okv0
From a computing perspective, the scenario depicted above demands a new class of microcontroller-class of devices, standard compute platforms used as \ac{IoT} end-nodes due to their low cost and high flexibility. In addition to more traditional tasks such as data acquisition and transmission, these devices must be enhanced with advanced computing capabilities to meet the latency, throughput and energy requirements of on-chip inference and training workloads of emerging \textit{TinyML} applications. %In particular, they must efficiently sustain intense integer workloads needed to run on-chip inference tasks, as well as to perform more costly floating-point computation to enable on-chip training and continual learning oriented applications. All within the typical power budget of battery-powered systems (few tens of milliWatts).

% Inference tasks -- quantization okv0
For inference tasks, the full-precision \ac{DNN} model is out-of-scale to fit the resources of IoT devices, nor is strictly required to satisfy the needs of \textit{TinyML} applications. Quantization-aware~\cite{jacob2018quantization} and post-training quantization techniques~\cite{hubara2017quantized} adopting low-precision integer arithmetic are well-established solutions to shrink the \ac{FP} \ac{DNN} model and deploy it on tiny IoT systems. In this domain, the mixed-precision approach~\cite{rusci2020leveraging}, where the activations and the weights of the \ac{DNN} are quantized asymmetrically, allows the model to fit the limited memory resources of microcontrollers, while reducing the Top-1 accuracy drop gap, compared to the full-precision \ac{FP} counterpart, within a 3 to 6\% range, acceptable for AI-enhanced \ac{IoT} applications. 

% Low-bitwidth integers in HW okv0
%Hence, low- and mixed-precision \acp{DNN} are one of the critical kernels to accelerate in extreme-edge devices. 
From an architectural viewpoint, low-bitwidth mixed-precision integer arithmetic has been mainly applied in digital specialized accelerators. Exploiting such data representation in dedicated hardware is very effective, as the design of the datapath is full custom and limited to a single or a subset of functions, safely tuning each operation to the desired precision with minimal overhead. Custom digital solutions like~\cite{lchen2019eyeriss, moons201714, ee2018unpu, desoli201714} achieve outstanding performance (1-50 TOPS/W) and energy efficiency (10-100 TOPS/W) on \ac{DNN} kernels. Recently this approach has been also adopted in analog-digital mixed-signal solutions~\cite{khaddam2022hermes, ueyoshi2022diana}, significantly boosting energy efficiency up to hundreds TOPS/W. However, these hardware units can only support operations with data precision for which they are designed for and the \ac{DNN} deployed model is strictly tight to the underlying architecture, with limited flexibility to evolve.

Enabling low-bitwidth mixed-precision computation on fully programmable architectures would ensure the highest flexibility in the kernels' data representation (to sustain different and evolving over time quantization schemes). However, applying this principle to processors is much more challenging, since the algorithms and the data precision to be executed are not known a priori. Consequently, multiple formats must be supported, increasing the complexity and the overheads of instruction fetch and decode stages. Lightweight solutions have appeared in the RISC-V ecosystem, introducing hardware-accelerated extensions for low-precision arithmetic within the \ac{ISA} of the processors with minimal area power and performance overheads. Authors of~\cite{garofalo2021xpulpnn} propose RISC-V SIMD sum-of-dot-product instructions and custom mac-load operations to achieve ASIC-like efficiency on symmetric \ac{DNN} convolutions. Other works~\cite{ottavi2020mixed} move forward implementing light-weight status-based mixed-precision computing support to a RISC-V processor, showing two orders of magnitude better efficiency than existing commercial microcontroller solutions.

% DEPTHWISE and DATA MARSHALING
Unlike previous generation of TinyML \ac{DNN} models, \ac{SoA} MobileNets feature much more heterogeneous workloads, with standard convolutions combined with point-wise and depth-wise kernels. Despite they have less computation complexity and less footprint, depthwise layers are not as computationally efficient as standard convolutions, due to their poor intrinsic data reuse~\cite{garofalo2022heterogeneous}. Due to these characteristics, they are intrinsically challenging to parallelize with the previously mentioned techniques. In the DNN processing pipeline, the Amdahl's effect moves soon toward depth-wise kernels which becomes the computing bottleneck, demanding new acceleration solutions. Likewise, data marshaling operations (e.g., low-bitwidth transpose) commonly used in \acp{DNN} are inefficient as they heavily rely on sub-byte swap operations.

% Heterogeneous Computing
Aware of the variety of \textit{TinyML} compute requirements, single accelerators alone can not afford to accelerate end-to-end AI-enhanced applications. Rather, heterogeneous computing a promising solution to deliver TinyML's required performance, efficiency and flexibility while coping with strict power and cost constraints~\cite{VEGA}: multiple programmable cores provide flexible and efficient execution for generic parallel kernels, while specialized hardware accelerators provide extra performance and efficiency boost on key kernels that dominate the computational workload.


% On chip training and custom datapaths
Contrarily to inference, on-chip training imposes more strict requirements on the data representation precision. Integer arithmetic can not be used, due to its limited dynamic range, and \ac{FP} formats are still dominant. Traditionally, single- and double-precision \ac{FP} formats have been used for training on high-performance platforms, but they are too expensive in terms of operation latency and energy to be used at the edge. To develop extreme-edge novel learning algorithms, a strong effort was recently made to adapt learning algorithms to lower-precision like \ac{FP}16 and \ac{FP}8~\cite{rodriguez2018lower, sun2019hybrid}, demonstrating no accuracy loss but massive gains in terms of computation complexity. Despite this achievement, \textit{TinyML} on-chip training workload is still 10-100$\times$ larger than inference~\cite{ravaglia2021tinyml} and the performance requirements remain very high. Accelerating these workloads with general purpose processors would require a massive number of cores, which would blow up the SoC's area and power consumption unacceptably. Hence, fixed-function custom designs still are the most suitable solutions to deliver significantly high performance within a TinyML compatible area and power budget.


% Our solution
In this work, we present \textsc{Darkside}, a \ac{PULP}-based~\cite{starwars, VEGA} heterogeneous computing \ac{SoC} that targets emerging TinyML inference and on-chip training applications.
We introduce four main innovations in \textsc{Darkside}: \textit{1)} RISC-V cores with advanced low-bitwidth mixed-precision integer computing capabilities; three dedicated hardware accelerators:  \textit{2)} a Depth-Wise convolution Engine (DWE), \textit{3)} a low-overhead DataMover for marshaling operations, and \textit{4)} a low-power Tensor Product Engine (TPE) for efficient \ac{FP}16 matrix multiplications.
The cores and accelerators are tightly integrated into a shared-L1 cluster to enable advanced hardware/software cooperation. The chip has been fabricated in TSMC 65nm technology and shows peak integer performance (2-bit) of 65 GOPS with an efficiency of 835 GOPS/W. On \ac{TPE}-accelerated \ac{FP}16 workloads, it achieves up to 18.2 GFLOPS and a peak efficiency of 300 GFLOPS/W at 2.6 GFLOPS, achieving peak performance and efficiency similar to 8-bit integer operations.


==> 01_v3_Introduction.tex <==
\section{Introduction}
% TinyML requirements -- inference okv0
Recently, the research effort to deploy \ac{ML} and \ac{DL} algorithms at the extreme-edge of the \ac{IoT}, usually referred to as Tiny Machine Learning (\textit{TinyML}), has reached outstanding results, making it possible to deploy complex \ac{DL} models on such tiny systems. As an example, MobileNets~\cite{sandler2018mobilenetv2} have rapidly become state-of-the-art compute workload used for classification and object detection inference tasks, but also employed as a flexible template for tasks not related to vision~\cite{cai2018proxylessnas,incze2018bird, zhang2019lightweight}. 

% TinyML -- training okv0
Besides, many AI-enhanced \ac{IoT} applications require the deployed \ac{DL} model to adapt to new data and scenarios in which they operate. Re-train the model on data-centers collecting on-field data from the distributed \ac{IoT} end-nodes and then re-upload it on the edge devices might be expensive in terms of latency and power costs. A common direction of TinyML is to rethink the deployed \ac{DNN} as a dynamic model that can improve and adapt itself by learning from new sensed data directly on the end-nodes. Recent progress in this research area concern \ac{DNN} model tuning, partial on-chip training~\cite{ravaglia2021tinyml} or unsupervised continual learning~\cite{ren2021tinyol}, which have been applied successfully to a wide range of \ac{IoT} applications, such as anomaly detection tasks~\cite{unknown}. 

% new generation of IoT devices okv0
%From a computing perspective, the scenario depicted above demands a new class of microcontroller-class of devices, the standard compute platforms used as \ac{IoT} end-nodes, due to their low cost and high flexibility. In addition to more traditional tasks such as data acquisition and transmission, these devices must be enhanced with advanced computing capabilities to meet the latency, throughput and energy requirements of on-chip inference and training workloads of emerging \textit{TinyML} applications. 

% Inference tasks -- quantization okv0
%For inference tasks, the full-precision \ac{DNN} model is out-of-scale to fit the resources of IoT devices. 
Quantization-aware~\cite{jacob2018quantization} and post-training quantization techniques~\cite{hubara2017quantized} adopting low-precision integer arithmetic are well-established solutions to shrink the \ac{FP} \ac{DNN} model and deploy it on tiny systems for inference tasks. In this domain, the mixed-precision approach~\cite{rusci2020leveraging}, where the activations and the weights of the \ac{DNN} are quantized asymmetrically, allows the model to fit the limited memory resources of microcontrollers, while reducing the Top-1 accuracy drop gap, compared to the full-precision \ac{FP} counterpart, within a 3 to 6\% range, acceptable for AI-enhanced \ac{IoT} applications. 

% Low-bitwidth integers in HW okv0
%Hence, low- and mixed-precision \acp{DNN} are one of the critical kernels to accelerate in extreme-edge devices. 
From an architectural viewpoint, low-bitwidth mixed-precision integer arithmetic has been mainly applied in digital specialized accelerators. Exploiting such data representation in dedicated hardware is very effective, as the design of the datapath is full custom and limited to a single or a subset of functions, safely tuning each operation to the desired precision with minimal overhead. Custom digital solutions like~\cite{chen2019eyeriss, moons201714, lee2018unpu, desoli201714} achieve outstanding performance (1-50 TOPS/W) and energy efficiency (10-100 TOPS/W) on \ac{DNN} kernels. Recently this approach has been also adopted in analog-digital mixed-signal solutions~\cite{khaddam2022hermes, ueyoshi2022diana}, significantly boosting energy efficiency up to hundreds TOPS/W. However, these hardware units can only support operations with data precision for which they are designed for and the \ac{DNN} deployed model is strictly tight to the underlying architecture, with limited flexibility to evolve.

Enabling low-bitwidth mixed-precision computation on fully programmable architectures would ensure the highest flexibility in the kernels' data representation (to sustain different and evolving over time quantization schemes). However, applying this principle to processors is much more challenging, since the algorithms and the data precision to be executed are not known a priori. Consequently, multiple formats must be supported, increasing the complexity and the overheads of instruction fetch and decode stages. Lightweight solutions have appeared in the RISC-V ecosystem, introducing hardware-accelerated extensions for low-precision arithmetic within the \ac{ISA} of the processors with minimal area power and performance overheads. Authors of~\cite{garofalo2021xpulpnn} propose RISC-V SIMD sum-of-dot-product instructions and custom mac-load operations to achieve ASIC-like efficiency on symmetric \ac{DNN} convolutions. Other works~\cite{ottavi2020mixed} move forward implementing light-weight status-based mixed-precision computing support to a RISC-V processor, showing two orders of magnitude better efficiency than existing commercial microcontroller solutions.

% DEPTHWISE and DATA MARSHALING
Unlike previous generation of TinyML \ac{DNN} models, \ac{SoA} MobileNets feature much more heterogeneous workloads, with standard convolutions combined with point-wise and depth-wise kernels. Despite they have less computation complexity and less footprint, depthwise layers are not as computationally efficient as standard convolutions, due to their poor intrinsic data reuse~\cite{garofalo2022heterogeneous}. For this reason, they are intrinsically challenging to parallelize with the previously mentioned techniques. In the DNN processing pipeline, the Amdahl's effect moves soon toward depth-wise kernels which becomes the computing bottleneck, demanding new acceleration solutions. Likewise, data marshaling operations (e.g., low-bitwidth transpose) commonly used in \acp{DNN} are inefficient as they heavily rely on sub-byte swap operations.

% Heterogeneous Computing
Aware of the variety of \textit{TinyML} compute requirements, single accelerators alone can not afford to accelerate end-to-end AI-enhanced applications. Rather, heterogeneous computing is a promising solution to deliver TinyML's required performance, efficiency and flexibility while coping with strict power and cost constraints~\cite{VEGA}: multiple programmable cores provide flexible and efficient execution for generic parallel kernels, while specialized hardware accelerators provide extra performance and efficiency boost on key kernels that dominate the computational workload.


% On chip training and custom datapaths
Contrarily to inference, on-chip training imposes more strict requirements on the data representation precision. Integer arithmetic can not be used, due to its limited dynamic range, and \ac{FP} formats are still dominant. Traditionally, single- and double-precision \ac{FP} formats have been used for training on high-performance platforms, but they are too expensive in terms of operation latency and energy to be used at the edge. To develop extreme-edge novel learning algorithms, a strong effort was recently made to adapt learning algorithms to lower-precision like \ac{FP}16 and \ac{FP}8~\cite{rodriguez2018lower, sun2019hybrid}, demonstrating no accuracy loss but massive gains in terms of computation complexity reduction. Despite this achievement, \textit{TinyML} on-chip training workload is still 10-100$\times$ larger than inference~\cite{ravaglia2021tinyml} and the performance requirements remain very high. Accelerating these workloads with general purpose processors would require a massive number of cores, which would blow up the SoC's area and power consumption unacceptably. Hence, fixed-function custom designs still are the most suitable solutions to deliver significantly high performance within a TinyML compatible area and power budget.


% Our solution
In this work, we present \textsc{Darkside}, a \ac{PULP}-based~\cite{starwars, VEGA} heterogeneous computing \ac{SoC} that targets emerging TinyML inference and on-chip training applications.
We introduce four main innovations in \textsc{Darkside}: \textit{1)} RISC-V cores with advanced low-bitwidth mixed-precision integer computing capabilities; three dedicated hardware accelerators:  \textit{2)} a \ac{DWE}, \textit{3)} a low-overhead DataMover for marshaling operations, and \textit{4)} a low-power \ac{TPE} for efficient \ac{FP}16 matrix multiplications.
The cores and accelerators are tightly integrated into a shared-L1 cluster to enable advanced hardware/software cooperation. The chip has been fabricated in TSMC 65nm technology and shows peak integer performance (2-bit) of 65 GOPS with an efficiency of 835 GOPS/W. On \ac{TPE}-accelerated \ac{FP}16 workloads, it achieves up to 18.2 GFLOPS and a peak efficiency of 300 GFLOPS/W at 2.6 GFLOPS, achieving peak performance and efficiency similar to 8-bit integer operations.


==> 02_Related_Work.tex <==
\section{Related Work}

==> 03_SoC_Architecture.tex <==
\section{Darkside SoC Architecture}

% ARCHI Figure
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{clean/Darkside_only_archi.pdf}
    \vspace{-2mm}
    \caption{ Overview of the \textsc{Darkside} cluster architecture, featuring 8 RVNN cores, the \ac{TPE}, the \ac{DWE} and the DataMover accelerators.}
    \label{fig:dark_archi}
    \vspace{-4mm}
\end{figure}

% IMAGE -- HW SW COOPERATION
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{clean/heterogeneous_example.pdf}
    \vspace{-2mm}
    \caption{\textsc{Darkside} heterogeneous operation. Figure shows a \ac{DNN} with 3 mixed-precision quantized layers and a final fully-connected layer using all the cluster blocks and communicating through software-managed buffers allocated on the shared L1 memory.}
    \label{fig:heterogeneous_example}
    \vspace{-4mm}
\end{figure}

% SOC DESCRIPTION -- INTRO 
Fig.~\ref{fig:dark_archi} shows the architecture of the \textsc{Darkside} cluster. It is built around eight 81kGE RISC-V-based 32-bit processors (\textit{RVNN} cores) and three specialized digital accelerators, the \textit{\ac{TPE}}, the \textit{\ac{DWE}} and the \textit{DataMover}\textcolor{red}{, which are designed to have reduced impact on the power and area metrics of the cluster.} The heterogeneous cluster can be used to support complex ML models, such as those depicted in Fig.~\ref{fig:heterogeneous_example}, through cooperation among its hardware compute units. The \textit{RVNN} cores feature a custom RISC-V \ac{ISA}, described in Sec.~\ref{sec:RV-NN}, while each accelerator, described in detail in the following subsections, is integrated using the \ac{PULP} \ac{HWPE} standardized interface\footnote{https://hwpe-doc.readthedocs.io}. Such an interface exposes to the rest of the cluster a \textcolor{red}{wide data transfer port (typically much higher than 32-bit)} to optimize the access to the SRAM L1 memory and a control port that allows the RISC-V cores to program the accelerator through memory-mapped control registers\textcolor{red}{, as visible in Fig.~\ref{fig:dark_archi}}. In each \ac{HWPE}, specialized internal \textit{Streamers} move data between the accelerators and the L1 memory through the data port, converting the memory accesses into data streams to feed the accelerator's datapath. 

% IMAGE -- RV-NN ARCHI AND ASSEMBLY
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{hci_rebuttal.pdf}
    \vspace{-2mm}
    \caption{Simplified example of HCI \textit{shallow} routing and arbitration between \textit{shallow} and \textit{logarithmic} branches, considering $N$ TCDM banks. The example shows a \textit{shallow} 128-bit (4-ports) wide access starting on bank 1 and two 32-bit accesses from the \textit{logarithmic} side.}
    \label{fig:hci_rebuttal}
    \vspace{-5mm}
\end{figure}

% HCI - TCDM
The cores and the accelerators share data on a scratch-pad 128 kB multi-banked L1 \ac{TCDM}, composed of 32 4-kB SRAM banks capable of serving 32 requests in parallel. The memory requests are routed through a one-cycle latency \ac{HCI}, leveraging a request/grant protocol and a world-level interleaving scheme to evenly distribute the requests, minimizing the access contentions toward the SRAM banks. 

The \ac{HCI} is organized in two branches, \textit{logarithmic} and \textit{shallow}, \textcolor{blue}{as shown in Fig.~\ref{fig:dark_archi}}: the cores, the cluster DMA and the DataMover access the L1 banks from the  \textit{logarithmic} branch through 9 32-bit initiator ports. This branch allows all-to-all single-cycle access from the initiator ports to each word interleaved memory bank. Conflicts are handled by granting one initiator per bank at the time through a round-robin scheme. The \ac{TPE} and the \ac{DWE} statically share a single wider initiator port (288-bit wide) in the \textit{shallow} branch, routed to 9 adjacent memory banks without arbitration. \textcolor{blue}{Considering a total of $N$ TCDM banks, routing works by splitting the address of the 288-bit wide word in an \textit{index} (bits $2$ through $\mathrm{log}_2(N)+2$) and an \textit{offset} part (upper bits). The index is used to select which TCDM banks are targeted, while the offset is used to compute the bank level address, considering the possibility that the wide word ``rolls over'' the set of banks (if the index corresponds to one of the last banks).}
On the memory side, the \ac{TCDM} banks are connected to the two \ac{HCI} branches via multiplexers, granting access to one branch or the other according to a configurable-latency starvation-free rotation scheme.
\textcolor{blue}{Ports from the logarithmic branch are stalled individually, whereas those from the shallow branch are stalled collectively (a single collision will result in no grant for the whole branch) to reflect the fact that they are actually a single access. Priority is given to a branch configurable via a memory-mapped register, and switched for a single access after a configurable number of cycles.
Fig.~\ref{fig:hci_rebuttal} showcases this mechanism in an example.}

This heterogeneous organization serves two purposes. On the one hand, the \ac{HCI} can be configured in software \textcolor{blue}{(by writing a memory-mapped register)} to prioritize either the \textit{shallow} or the \textit{logarithmic} branch and guarantee a minimum quality of service (in terms of consecutive stall cycles) to the non-priority branch \textcolor{blue}{ (by setting a register with the maximum number of stalls that the less priority branch can tolerate)}. This enables to control and tune the interconnect performance at a fine granularity. \textcolor{blue}{For example, setting priority to the \textit{shallow} branch and maximum stall of 10 cycles in the \textit{logarithmic} branch means that after 10 collisions the priority will be switched to \textit{logaritmic} side for one cycle, hence guaranteeing a 9.1\% collision rate, delivering up to 37.1 GB/s at 290 MHz even on data-intensive kernels.}

On the other hand, the scalability of the \textit{logarithmic} interconnect is limited:  attaching the accelerators to a non-hierarchical interconnect would result in a much more complex, larger, and power-hungry interconnect circuit, leading to poor cluster-level performance-per-area and per power. 
The \ac{HCI} occupies 7.3\% ($\sim$220kGE) of the total cluster area; \textcolor{blue}{our synthesis trials have shown that the overall the complexity of the interconnect is reduced by 15\% with respect to a purely logarithmic interconnect, which combined with easier timing closure and extended functionality led to the choice of this design}.

% DMA -- I$ -- EVENT UNIT
The cluster also features a two-level hierarchical instruction cache (I\$), implemented with latch-based SCM to improve the energy efficiency over energy-expensive SRAM cuts. It includes 8 512-B private per-core plus 4kB of two-cycle shared cache to maximize the efficiency with the data-parallel code. A dedicated DMA controller, featuring a similar size as the cores ($\sim$84 kGE), efficiently manages the data transfer between the L2 (off-the-cluster) and L1 memory. The DMA supports 2-D data transfers and up to 16 outstanding transactions, hiding the latency of L2-L1 data transfers on data-intensive kernels~\cite{burrello2021dory}, while saving energy compared to cached-based systems. Fine-grained parallel thread dispatching is accelerated by a Hardware Synchronization Unit ($\sim$30 kGE), which also manages clock-gating of idle cores waiting for synchronization. % and enables resuming the execution in two cycles.The cluster is also supported by a small Hardware Synchronization Unit (~30 kGE) that manages synchronization and thread dispatching, enabling low-overhead and fine-grained parallelism, thus high energy efficiency.

% SOC -- TESTBENCH
The cluster resides in a dedicated power and clock domain. It is surrounded by other IPs integrated into a different power and clock domain, namely the \textit{Fabric} domain. The latter includes a controlling RISC-V processor, FLLs for clock generation, a standard set of I/O peripherals and 256 kB of L2 memory containing the code executed by both the compute cluster and the controlling RISC-V core. In the context of this work, the \textit{Fabric} domain serves as a programmable testbench for the cluster, which is the main architectural contribution of this work. The communication bus between the \textit{Fabric} and the cluster domain is AXI4 based, and dual clock first-in-first-out (FIFO) buffers are used for clock domain crossing.

\subsection{Dynamic Bit-Scalable Fused Mac-Load SIMD Operations}
\label{sec:RV-NN}

% IMAGE -- RV-NN ARCHI AND ASSEMBLY
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{ri5cy_nn-darkside_v3.pdf}
    \vspace{-2mm}
    \caption{a) Pipeline extension to the core to support the M\&L instruction.  b) Example of a  \textit{MatMul} kernel with M\&L instruction. Thanks to the M\&L operating on the dedicated NN-RF, we can implement larger structures of \textit{MatMul} kernels (right-sided) with a significant gain in terms of throughput.}
    \label{fig:riscy_nn}
    \vspace{-5mm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%
%%%%%%%%%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%
%%%%%%%%%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%
%%%%%%%%%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%%V1%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% RV-NN CORE EXTEND MPIC - INTRO
%The cores of the \textit{Darkside} cluster, namely RV-NN, enhance the 32-bit RISC-V processor presented in~\cite{ottavi2020mixed}, namely MPIC, by extending its \ac{ISA} and optimizing its micro-architecture. The MPIC core features the RV32IMCxPULP~\cite{gautschi2017near} \ac{ISA} extended with 2-bit to 32-bit custom mixed-precision SIMD instructions, suppored through a status-based execution. The SIMD instructions include \textit{dot-product (dotp)} based SIMD operations, relevant to speed-up low-bitwidth compute-intensive kernels like Matrix-Matrix and Matrx-Vector multiplications.

% M&L -- INTRODUCE M&L AND ASSEMBLY IMPROVEMENTS
%The key enhancement we propose to the MPIC core is a fused MAC-load (M\&L) operation to reduce the load overheads within the innermost loops of compute-intensive kernels.
%
%The intuition behind the design of the M\&L comes from the memory access pattern regularity of Matrix-like operations; while we consume current operands with a MAC operation we can fetch already the next operands by offsetting the current memory address pointer by a known value. Therefore, we can collapse the MAC and the Load operation within a single instruction, since the datapath activated by the MAC operation would not interfere with the Load-Store Unit of the processor. From an instruction perspective, the advantages of the designed M\&L are shown in Fig.~\ref{fig:riscy_nn}b. After out-of-the-loop initialization of a dedicated Neural \ac{NN-RF} on which the M\&L operates, we perform 8 \textit{dotp}-like operations at the cost of only one explicit load, with an instruction/cycle improvement of {{57\%}} compared to the MPIC baseline. 

% M&L -- uARCHI EXTENSION
%To support the M\&L within the RVNN micro-architecture, we extend its datapath to fuse one load and one \textit{dotp}-based SIMD operation in one single-cycle latency instruction, as shown in Fig.~\ref{fig:riscy_nn}a. The M\&L instructions fetch the source operands of the \textit{dotp} from the dedicated \ac{NN-RF}, while the accumulators reside in the \ac{GP-RF}. When a M\&L instruction is executed, one of the two source operands from the \ac{NN-RF} can be updated with new data fetched from the memory by the LSU of the core, that is extended to operate also on the \ac{NN-RF}. The registers of the \ac{NN-RF} are allowed to be kept static until necessary, by using a second M\&L instruction encoded into the \ac{ISA} that performs only the \textit{dotp} branch, but still fetch its operands from the \ac{NN-RF}. This allows a higher grade of flexibility for data reuse strategies, commonly used on resource constraint devices to increase the computation efficiency on compute intensive kernels. With this strategy, data reuse is not limited by the compiler scheduler on the time we can keep an operand into the \ac{GP-RF}. This flexibility comes without sacrificing the programmability, as we extend the RISC-V gcc toolchain to support the M\&L instructions, so that it can be inferred into the C code through built-ins. 

% M&L --  IMPACT ON PPA OF MPIC
%The M\&L extension loosely impacts the Performance, Power, Area (PPA) metrics of the RVNN core: it implies a gate count increase of just {{8.3\%}}, without deteriorating the critical path of the core and with negligible power overhead. On the contrary, the core enhanced with the M\&L achieves up to {{91\%}} MAC utilization, compared with {{58\%}} of the MPIC baseline. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%
%%%%%%%%%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%
%%%%%%%%%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%
%%%%%%%%%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%%V2%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RV-NN CORE EXTEND MPIC - INTRO --> V2
The \textit{Darkside} cluster's core, namely RVNN, is a 4-stage in-order single-issue pipeline, \textcolor{red}{depicted in Fig.~\ref{fig:riscy_nn}a,} that implements the RV32IMCF RISC-V \ac{ISA}, plus custom mixed-precision SIMD instructions \textcolor{red}{operating on vector elements with power-of-two precision formats from 2-bit to 32-bit and all their possible permutations}, supported through a \textcolor{red}{dynamic bit-scalable} execution~\cite{ottavi2020mixed}. The SIMD instructions include \textit{dot-product (dotp)} based operations relevant to speed-up low-bitwidth compute-intensive kernels like Matrix-Matrix and Matrix-Vector multiplications. The micro-architecture to support the mixed-precision operations and the \textcolor{red}{dynamic bit-scalable} execution is built on top of the RI5CY~\cite{gautschi2017near} core; \textcolor{red}{to minimize the logic necessary to implement the new extensions, the first operand of the mixed-precision operations is designated to be always the highest precision operand, without loss of generality given the commutative property of add and multiply operators. The extended pipeline entails 17\% area overhead and 3\% power overhead compared to RI5CY, but it improves the performance on sub-byte and mixed-precision kernels by a significant factor (up to 7.7$\times$). }


% M&L -- INTRODUCE M&L AND ASSEMBLY IMPROVEMENTS -- V2
%  \textbf{and the addresses for the memory accesses in the Control Status Registers (CSRs)}
The key enhancement of RVNN is a fused MAC-load (M\&L) operation that applies to any mixed-precision SIMD \textit{dotp} instruction supported. The design of the M\&L collapses the SIMD MAC and the load operations into a single one-cycle latency instruction since the datapath activated by the MAC operation would not interfere with the Load-Store Unit of the processor, and the two units can run in parallel. Fig.~\ref{fig:riscy_nn}a shows the micro-architectural modifications to the cores' datapath to enable the M\&L. The M\&L fetches the two operands for the \textit{dotp} operation from a dedicated register file, namely the Neural Network Register File (NN-RF), consisting of 6 32-bit registers. At the same time, the accumulators reside in the GP-RF. 

\textcolor{red}{The NN-RF is sized to maximize the innermost loops performance of the PULP-NN~\cite{garofalo2020pulp} convolution routines, dedicating 4 out of 6 registers to layer's weights and 2 out of 6 registers to input activations. In mixed-precision \textit{sdotp} operations, this choice constraints the activations of the convolution layers always to feature higher precision than the weights, which however is always the case in current state-of-the-art software solutions to deploy \ac{DNN} models at the extreme-edge of the IoT~\cite{rakka2022mixed}. The integration of the NN-RF in the \textsc{EX-STAGE} of the core costs only 5\% of area overhead}. Still, it reduces the occupancy of the 32 registers of the \ac{GP-RF} by a significant factor since it would host only the accumulators, leaving space for the implementation of kernels with a higher amount of data reuse (Fig.~\ref{fig:riscy_nn}, right-sided kernel). When a M\&L instruction is executed, one of the two source operands from the \ac{NN-RF} can eventually be updated with new data fetched from memory by the LSU,  extended to operate on the \ac{NN-RF} with negligible area overhead. However, the data stored in the \ac{NN-RF} registers can be kept until necessary to allow a higher degree of flexibility for data reuse strategies: a second M\&L instruction encoded into the \ac{ISA} performs only the \textit{dotp} branch, with no register update. 


%
From an instruction count perspective, the M\&L brings significant advantages, as shown in Fig.\ref{fig:riscy_nn}b. After out-of-the-loop initialization of the dedicated Neural \ac{NN-RF}, we perform 16 SIMD \textit{dotp}-like operations and only a single explicit load (with no concurrent MAC) instruction. Therefore, we reduce the number of pure load instructions in the innermost loop of the kernel by a factor of 6, at the same time doubling the throughput, with an overall dot-product/cycle improvement of {{57\%}} compared to the same core not featuring the M\&L. On the contrary, the impact of the M\&L on the Performance, Power, and Area (PPA) metrics of the RVNN core is minimal. Overall, the M\&L implies a gate count increase of just {{8.3\%}}, without deteriorating the critical path of the core and with negligible power overhead. On the other hand, the core enhanced with the M\&L achieves up to {{94\%}} dot-product unit utilization, compared with {{58\%}} of the RI5CY baseline.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{TPE_Scheduling_Diagram.pdf}
    \vspace{-2mm}
    \caption{Architecture of the \ac{TPE}, with a focus on the interconnection  of the FMAs within the datapath.}
    \vspace{-4mm}
    \label{fig:tpe_detail}
\end{figure}

\subsection{Tensor Product Engine}
\label{sec:TPE_archi}
The Tensor Product Engine (\ac{TPE})~\cite{redmuledate2022} accelerates matrix multiplications (MatMuls) of the kind $ Z\;= X \cdot W$. It is designed to use the IEEE 754 binary-16 representation (FP16 in the following) since it is understood that \ac{FP}16 can be used to train Neural Networks without significant accuracy loss, but reducing the power consumption and time to computation \cite{nvidia_mixp}.
%
Fig.~\ref{fig:tpe_detail} shows the implementation of the \ac{TPE}. The datapath consists of 32 \ac{FP}16 \ac{FMA} units~\cite{tagliavini2018transprecision} organized in 8 rows, each of 4 columns. This configuration guarantees at the same time a good speed-up (from $9\times$ up to $22\times$) with respect to the software parallel execution, and an area overhead bounded to 44.8\% of the area occupied by all the RV-NN cores.
%
The \acp{FMA} along each row are cascaded; each \ac{FMA} passes the intermediate result as input to the unit to its right. 

% NEW PARAGRAPH 
To internally handle the computation of matrices larger than the array size, and to avoid intermediate store operations, the \acp{FMA} in each row are closed in a feedback loop so that the right-most \ac{FMA} feeds back the computed partial product as accumulation input to the left-most \ac{FMA} of the same row. Using this approach, the \ac{TPE} can exploit maximum reuse of both the \textbf{X}-matrix elements and the intermediate product, so that it stores the computed sub-blocks of the \textbf{Z}-matrix to the memory only at the very end of their computation.
%
To match the critical path of the cores, each \ac{FMA} features three internal pipeline registers. To maximize throughput, the \textbf{X}-matrix elements of each \ac{FMA} are held steady for the number of cycles necessary to the \acp{FMA} of each row to compute the partial results. On the other hand, \textbf{W}-matrix operands are streamed-in at each cycle and broadcasted to all the \acp{FMA} of the same column.
The memory accesses are scheduled so the load and store phases do not introduce overhead during the computation. This way, the \ac{TPE} can reach an overall 98.8\% utilization of the internal \acp{FMA} with a near-to-ideal performance (31.6 out of 32 MAC/cycle).
The computed sub-blocks of the \textbf{Z}-matrix are stored in the memory only at the end of their computation, maximizing internal data reuse. 

\textcolor{red}{The \ac{TPE}, as well as the other accelerators integrated in Darkside, features a non-blocking event-based execution mode: the cores of the cluster, after programming the accelerator and starting its execution, can either go in sleep mode or resume software code execution. This mechanism enables complex execution models where the accelerator can be used in parallel with the general-purpose cores to boost the performance of the target kernel. }\textcolor{red}{When not used for FP16 Matrix operations, the TPE goes in fully clock-gated idle state to save power.}

\subsection{Depth-Wise Convolution Engine}
\label{sec:DWE_archi}

%% IMAGE -- DEPTHWISE ACCELERATOR
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{clean/DWE.pdf}
    \vspace{-2mm}
    \caption{(a) Architecture overview of the Depth-wise digital accelerator, enclosed in the HWPE. (b) Execution flow of the depth-wise operation.}
    \label{fig:dwe_archi}
    \vspace{-4mm}
\end{figure}

% DWE -- INTRO
The Depth-Wise Convolution Engine (\ac{DWE}) can process the low-reuse depth-wise component of the depth-wise + point-wise kernels often used in recent neural network models for mobile applications, leaving the much better-parallelizable point-wise kernels to the M\&L-accelerated software. The \ac{DWE} processes 8-bit signed input and weight tensors stored in L1 memory using the \ac{HWC} layout, the same used by the cores to execute the point-wise kernels and therefore requiring no time-consuming intermediate on-the-fly marshalling operations. The 8-bit output tensors are generated after applying re-quantization steps. %and generates 8-bit output tensors after re-quantization steps. %The \ac{DWE} is designed to work on input and output tensors stored in memory using the \ac{HWC} layout. This design choice is advantageous because it is the same layout used by the cores to compute the point-wise layers. Therefore  no additional on-the-fly data marshalling operations are required.

%  DWE -- WEIGHT BUFFER
The architecture is shown in Fig.~\ref{fig:dwe_archi}a. It employs a weight-stationary data flow to maximize the data reuse and targets 3$\times$3 depth-wise layers, the one most commonly encountered in \acp{DNN}. \textcolor{red}{Although its datapath is optimized for 3$\times$3 depth-wise convolutions, the DWE can be used to run kernels with different sizes using the same approach presented in~\cite{meloni2018neuraghe}, at the cost of additional data manipulation on the intermediate results, hence less computation efficiency.}

The execution flow is depicted in Fig.~\ref{fig:dwe_archi}b. The weights from 16 3$\times$3 filters are loaded into the \textit{Weights Buffer} \circled{1}, before the execution starts. The weights are kept in the buffer until they have been used to scan the whole input tensor. 
%
The input image is filtered through a vertical sliding window on the spatial dimensions, using a \textit{window buffer} of 4$\times$3$\times$16 registers. The first three rows are loaded at the beginning of the iteration \circled{2} and consumed in 4 cycles by the datapath of the \ac{DWE} consisting of 36 MAC units. The intermediate results are accumulated over 16 32-bit buffers, accessed 4 at a time in the 4-cycle operation loop \circled{3a}. Afterwards, non-linear activation functions and ancillary operations such as shifting and clipping are applied to re-quantize the results to 8-bit precision \circled{4}. After 4 cycles of operation, the 16-channel 8-bit pixels stored in the \textit{output buffer} are streamed out of the accelerator \circled{5}. Meanwhile, the streamer uses three cycles (overlapped with the computation) to fill the fourth row of the \textit{window buffer} \circled{3b}, needed to implement the sliding window mechanism.

The \ac{DWE} is designed to keep the datapath always active, in all stages and to fully exploit the memory bandwidth of 36B per cycle available on the cluster, achieving the overall performance of 30 MAC/cycle, more than 10$\times$ better than a software execution of the depth-wise kernels, on the 8 RVNN cores. \textcolor{red}{To save power when the accelerator is idle, the hardware block is fully clock gated, with negligible area overhead.}

%The datapath includes 36 MAC units which implement 3$\times$3 kernels which operate on 4 channels simultaneously. 
%The weights from 16 filters are loaded from the L1 memory and stored into the \textit{weight buffer} that features 16$\times$ 3$\times$3 registers. To maximize the data reuse, the weights reside in the buffer until they have been used to scan the whole input tensor. 

% DWE -- WINDOW BUFFER
%The input image is filtered using a vertical sliding window on the spatial dimensions, considering 16 channels of data stored in memory with the \ac{HWC} layout in each iteration. The sliding mechanism is implemented utilizing a \textit{window buffer} of 4$\times$3$\times$16 registers. The first three rows of the \textit{window buffer} are consumed in 4 cycles of operation of the MAC units. Every 4 cycles of operation, the streamer uses 3 cycles (overlapped to the computation) to load the next 16-channel input image pixels needed to implement the spatial sliding window mechanism over the input image. The data flow and consequently the architecture of the \ac{DWE} datapath is designed to fully exploit the memory bandwidth of 16B per cycle available on the cluster, achieving the overall performance of 30 MAC/cycle, 26$\times$ better than a software execution of the depth-wise kernels, on the 8 RVNN cores.

% DWE -- OUTPUT BUFFER
%The intermediate results are accumulated over 16$\times$ 32-bit registers, accessed 4 at a time in the 4-cycle operation loop. Afterwards, non-linear activation functions and ancillary operations such as shifting and clipping are applied to re-quantize the results to 8-bit precision.
%In the last cycle of the 4-cycle operation loop, the 16-channel 8-bit pixel is streamed out of the accelerator.

\subsection{DataMover}
\label{sec:datamover}
%% IMAGE -- DATAMOVER ARCHI 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{clean/DataMover_archi.pdf}
    \vspace{-2mm}
    \caption{Overview of the DataMover architecture and execution flow.}
    \label{fig:datamover}
    \vspace{-1mm}
\end{figure}
%On-the-fly data marshalling operations can dramatically reduce the performance of \ac{DNN} workloads, during both inference and training tasks. 
To perform efficiently on-the-fly data transposition, the \textit{Darkside} cluster is enhanced with a DataMover unit, exposed to the \ac{HCI} with an additional master port on the \textit{logarithmic} branch. The architecture is depicted in Fig.~\ref{fig:datamover}. It consists of a tiny accelerator of only 54 kGE, capable of transposing \ac{DNN} 3-dimensional tensors stored in the L1 memory, with 1.5-100$\times$ less time than eight RVNN cores and increased energy efficiency up to 50$\times$ (the lower the precision of chunks to transpose the more significant the advantages).% power consumption which is on average ~50\% lower than the cores. %Similar to the cores, the DataMover has a dedicated master port on the \textit{logarithmic} branch of the \ac{HCI}.

The accelerator works on data with configurable precision, $d$, in the range from 32-bit down to 1-bit. It splits incoming data streams from memory into chunks of size $d$, internally buffered into the \textit{Shuffle Buffer} which features 32$\times$ 32-bit register with the transposed output format; only 32/$d$ of them are used, depending on the data size configuration $d$. After 32/$d$ input stream transactions, the transposed words are streamed out to the L1 memory and the accelerator continues the operations with new input streams. \textcolor{red}{When data transposition is not requested, the accelerator goes in a clock-gated idle state to reduce its impact on to the total power consumption of the cluster.}



==> 05_Benchmarking.tex <==
\section{Benchmarking}
% intro
To demonstrate the computing capabilities of \textsc{Darkside} on \ac{SoA} DNN workloads, we benchmark mixed-precision convolution kernels, end-to-end inference of the MobileNetV2 and one TinyML training use-case.
%\textsc{Darkside} is designed to computationally sustain the heterogeneous workloads of \ac{SoA} DNN models. In this section we benchmark mixed-precision convolution kernels, the end-to-end inference task of the MobileNetV2 and one training use-case.

%To demonstrate the benefits of the proposed heterogeneous compute fabric,
\subsection{Single DNN Kernels}

% IMAGE -- mixed-precision kernels, normalized perf
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Normalized_performance_v4.pdf}
    \vspace{-4mm}
    \caption{Left: Normalized single-core performance of mixed-precision convolutions. RVNN core (\textit{Mixed w M\&L}) is compared against a core featuring only mixed-precision \textit{dotp} operations but no M\&L (\textit{Mixed}) and against \textit{RI5CY}, which features no extensions for quantized neural networks. Right: performance improvement of execution on cluster-coupled accelerators over software (8-cores).}
    %\caption{Left: Normalized single-core performance of quantized DNN kernels. \textsc{Darkside}'s core performance is compared with Dustin's \cite{ottavi2022dustin} and Vega's core \cite{VEGA}. Right: performance improvement of execution on cluster-coupled accelerators over software (8-cores).}
    \label{fig:normalized_perf}
    \vspace{-4mm}
\end{figure}

% INTEGER DNN KERNELS
To highlight the features of the RVNN cores, we incrementally show the improvements over the baseline, benchmarking several convolution kernels. To measure the computing performance, the layers operate on data stored in the L1 memory, with 64 3$\times$3$\times$32 filters applied on a 32$\times$16$\times$16 input feature map, spanning different integer data formats (from 8- down to 2-bit) for the inputs and the weights, including mixed-precision cases. The results are reported in Fig.~\ref{fig:normalized_perf} in terms of normalized execution cycles (with respect to the RVNN core with the M\&L). As shown, the M\&L instruction improves the performance by up to 1.7$\times$ comparedthe execution with separated mixed-precision SIMD \textit{dotp} and load instructions (\textit{Mixed} in the figure). Overall, our ISA and micro-architecture design of RVNN leads to a cumulative performance improvement of up to 13$\times$ with respect to RI5CY, which supports only 8-bit SIMD operations and no M\&L mechanisms. 

% DEPTHWISE KERNELS
Analyzing the depth-wise kernels, in Fig.~\ref{fig:normalized_perf} we show that this workload would benefit at least 5.8$\times$ better performance by offloading it to the dedicated digital accelerator presented in this work, the Depth-wise engine (\textit{DWE}), instead of performing the depthwise on 8 RVNN cores. This conclusion is also remarked in Sec.~\ref{sec:end_to_end_inference} on a real-sized \textit{Bottleneck} layer use-case. As a final analysis, we show that the DataMover can save more than 3.7$\times$ execution cycles on 8-bit data marshalling operations, compared to the same task offloaded to the 8 cores.% of the cluster.
%The depth-wise convolutions are other fundamental DNN kernels commonly used in modern DNN topologies. Due to their lower intrinsic data reuse compared to standard convolution layers, it is hard to reach good performance for this workload on embedded general-purpose cores: the execution of the kernel would require a non-negligible amount of data manipulation instructions against few dot-product operations to perform, lowering the operation efficiency of the cores. Therefore, in Fig.~\ref{fig:normalized_perf} we show that this workload would benefit at least 5.8$\times$ better performance by offloading it to the dedicated digital accelerator presented in this work, the Depth-wise engine (\textit{DWE}). This conclusion is also remarked in Sec.~\ref{sec:end_to_end_inference} on a real-sized \textit{Bottleneck} layer use-case. As a final analysis, we show that a small accelerator like the DataMover can save more than 3.7$\times$ execution cycles on 8-bit data marshalling operations, compared to the same task offloaded to the cores of the cluster.

% FP 
On 16-bit floating-point (FP16) matrix-multiplication workloads, the TPE boosts the performance by up to 10.3$\times$ with respect to the software execution of the same kernels exploiting the FP16 SIMD instructions available on the 4 floating-point units (FPUs) present in the cluster~\cite{tagliavini2018transprecision}. 

\subsection{End-to-End MobileNetV2}
\label{sec:end_to_end_inference}
%As a representative workload for DNN inference we select the MobileNetV2~\cite{sandler2018mobilenetv2}: a widely used network topology for computer vision on mobile devices, both for classification and object detection, but also employed as a flexible template for tasks not related to vision~\cite{cai2018proxylessnas,incze2018bird, zhang2019lightweight}. The workload of this DNN model is highly heterogeneous, with depthwise convolutions, residuals, activation functions that evolve fast and other building blocks combined with standard convolutions.

%
First, we present the results of benchmarking the \textit{Bottleneck} layer, the core building block of the MobileNetV2. We demonstrate our improvements incrementally by comparing our architectural solutions over a reference cluster that features 8 RI5CY cores (without the mixed-precision SIMD operations and the M\&L custom ISA extensions proposed in this work) and no dedicated accelerator.
To implement the software to execute the \textit{Bottleneck} we use the PULP-NN library (which we use as-is to benchmark the reference cluster), extended to include additional kernels to exploit the new ISA instructions implemented in the RV-NN cores and a set of hardware-abstraction-layer (HAL) functions to program and start the accelerators that the programmer can easily insert into the C code. We adopt the 8-bit signed integer representation for all the tensors of the \textit{Bottleneck}.

% IMAGE -- Bottleneck layer results
% : in the \textit{SW RI5CY} configuration (our baseline), both the PWs and the DW layers are offloaded to the RISC-V cores, which do not feature the ISA extensions presented in this work; in \textit{SW RV-NN}, all the layers are executed on the RV-NN cores, while in \textit{SW RV-NN \& Datamover} the HWC to CHW marshalling operation is performed by the DataMover. Finally, in \textit{SW RV-NN \& DWE}, PWs are offloaded to the cores, DW to the Depth-wise Engine (DWE) accelerator; in this case there is no need for any marshalling operation.
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{Bottleneck_layer.pdf}
    \vspace{-2mm}
    \caption{Comparison of the \textit{Bottleneck} layer execution, offloaded to different hardware compute units. a) reports the execution latency (in terms of compute cycles), b) reports the energy efficiency (in GOPS/W). The cluster is running at the best performance operating point: $f_{CLU}\,=\,290\,MHz$, $V_{DD}\,=\,1.2\,V$.}
    \label{fig:bottleneck_results} 
    \vspace{-2mm}
\end{figure}

% bottleneck results
The results, in terms of execution cycles and energy efficiency, are reported in Fig.~\ref{fig:bottleneck_results}. The M\&L improves the execution of point-wise and depth-wise layers on 8 RVNN cores by 1.31$\times$ compared to the execution on 8 RI5CY cores. Additional 1.13$\times$ improvements are given by the data transposition (i.e. HWC to CHW data marshalling) performed by the DataMover, instead of transposing data via software. Finally, the DWE allows to speed-up the execution of depth-wise convolution by 4.4$\times$ compared to the execution on 8 RV-NN cores, with a final performance improvement of 1.85$\times$ on the whole \textit{Bottleneck} layer compared to the RI5CY baseline.


% end-to-end mobilenet
To put the previous results in perspective, we benchmark \textsc{Darkside} on the end-to-end inference task of the MobileNetV2 model. We employed the standard MobileNetV2 with depth multiplier 1.0 and input size 224$\times$224, composed of 16 stacked \textit{Bottleneck} layers. The input and weight tensors feature 8-bit precision for all the depth-wise and Conv2d layers. The point-wise layers feature 8-bit input tensors, while the weights are represented with reduced precision, i.e. 4-bits. This mixed-precision configuration of the model achieves similar Top-1 accuracy (only a 2.5\% drop compared to the 8-bit version) while ensuring almost 2$\times$ less memory footprint \textcolor{red}{(1.07 MB)} for the network weights~\cite{schaefer2022edge}. 

% IMAGE -- DARKSIDE DATA FLOW
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Darkside_Data_flow.pdf}
    \caption{DNN tiling software pipeline. The figure shows the concurrent execution of weights and activations transfer (from  L2 to  L1 memory, indicated with \textbf{\textit{IN}}), the computation of the kernel (indicated with \textbf{\textit{C}}) and the copy of produced output tiles from  L1 to  L2 memory (indicated with \textbf{\textit{O}}).}
    \label{fig:sw_pipe}
    \vspace{-3mm}
\end{figure}

% execution model
To enable the computation on the cluster, both  weights and  activations of the model must be divided into tiles that fit 128 kB of the L1 SRAM. Therefore, we assume the weights and the feature maps for all the network layers to be stored in the off-the-cluster L2 memory, and we adopt the data and execution flow presented in Dory~\cite{burrello2021dory}. Dory is used to calculating the data tiling solutions fitting the L1 memory constraints and to schedule the data transfers from L2 to L1 and vice-versa, performed through the cluster DMA in double-buffering. The described software pipeline is represented in Fig.~\ref{fig:sw_pipe}. For cases where the execution is not memory-bound, data movements overlap with the computation, with negligible overhead ($\leq 5\%$) to the execution latency.

% Description of the methodology
However, since \textsc{Darkside}'s \textit{Fabric} domain has the only purpose of acting as a programmable testbench for the cluster, its L2 memory is insufficient to host the entire MobileNetV2. Without loss of generality for our analysis, which aims at benchmarking the computing capabilities of \textsc{Darkside}'s cluster, we perform the experiments by building a model from the following measurements and considerations:
\begin{enumerate}
    \item \textcolor{red}{We assume to have an L2 memory of 2 MB to host the entire MobileNetV2 model and to store the program code;}
    \item We analyze the traffic between L2 and L1 memories by running simulations of the MobileNetV2 on an event-accurate simulator called GVSOC~\cite{bruschi2021gvsoc}, where we included the hardware description of the \textsc{Darkside} cluster and the \textit{Fabric} domain with \textcolor{red}{2MB of L2 memory}; as expected, during the execution of the inference task we are never memory-bound; therefore, the contribution of the L2 to L1 (and vice-versa) data movements is relevant only for the total energy consumption;
    \item We measure the latency and the energy of all the L2 to L1 data transfers (and vice-versa) necessary to compute each tile on the silicon prototype; 
    \item We measure the latency and the energy necessary to compute each tile generated by the Dory framework on the silicon prototype.
\end{enumerate}

% IMAGE -- MBNTv2 mixed 4-8 results
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{MBNTv2_mixed_4_8.pdf}
    \vspace{-2mm}
    \caption{Layer-wise execution latency and energy of the MobileNetV2 on \textsc{Darkside}'s cluster running at $f_{clk}=290\,MHz$ and $V_{DD}=1.2\,V$.}
    \label{fig:mbntv2}
    \vspace{-3mm}
\end{figure}
The layer-wise compute time and energy of the inference task are shown in Figure~\ref{fig:mbntv2}. \textsc{Darkside} can perform the entire end-to-end task with a performance of more than 20 frame/s, with an energy budget of 11mJ. The performance is 2$\times$ better than the one achieved on the Vega's cluster running at 250 MHz~\cite{VEGA}, thanks to our architectural contributions, the M\&L extensions that accelerate the point-wise kernels and the dedicated DWE that boosts the execution of depth-wise convolutions. Despite Vega being implemented in the 22nm technology node, our end-to-end energy consumption of 11 mJ remains still comparable, in the same order of magnitude.

%Thanks to the mac-load extensions and the mixed-precision support of the RV-NN core, to the dedicated depth-wise engine and a tighly-coupled architecture of the cluster, the entire task is executed with a performance of more than 20 frame/s within 11 mJ of energy budget, better and comparable, respectively, to the execution of the same DNN model on a similar cluster architectural template implementation in a much more scaled technology node CITE VEGA.

% TRAINING -- ok v0.1
\subsection{TinyML On-Chip Training}
The \ac{TPE} enhances the \textsc{Darkside} cluster to support efficient \ac{FP} matrix-matrix multiplications, enabling de-facto on-chip TinyML training workloads. To benchmark the \ac{SoC} in terms of execution latency and energy on real-sized problems, we execute the \ac{AE} \ac{DNN} model~\cite{unknown}, commonly used within the TinyML scenario for unsupervised anomaly detection tasks. The TinyML \ac{AE} consists of Encoder and Decoder layers (made by 128 unit Fully Connected layers with BatchNorm and ReLu activation functions) and a latent space layer of size 8. The input and the output size is 640. We benchmark the whole training stage (forward and backward steps within one training \textit{epoch}), adopting a batch size of 16, which is a reasonable trade-off between performance and memory occupation for \ac{IoT} multi-core microcontroller-class devices. The tensors are represented with the \ac{FP}16 format, and we adopt the same data flow explained above, which uses tilings and double-buffering.% techniques implemented with the cluster DMA for fast and efficient data movements.  

% Setup
To highlight the boost given by the \ac{TPE} and the DataMover, we first implement the \ac{AE} on the 8 general-purpose RVNN cores (we call this configuration \textit{SW}), which share 4 floating-point units supporting \ac{FP}16 formats, using a software library optimized for on-chip training~\cite{nando2022samos}. Then, we implement the \ac{AE} offloading the matrix-multiplication workload to the \ac{TPE} (\textit{TPE} configuration), still performing on the cores control tasks (e.g. programming the DMA for double buffering, programming the \ac{TPE} control units) and matrix transpositions. As a third execution mapping, we use the DataMover to speed-up also the matrix transpositions (\textit{TPE + DataMover}). 

% Training Results
\begin{figure}[t]
    \centering
    \includegraphics[width=0.88\linewidth]{AutoEncoder.pdf}
    \vspace{-2mm}
    \caption{a) Layer-wise execution time of the AutoEncoder (AE) TinyML model. b) Execution Energy of the AE, including the energy for L2 to L1 (and vice-versa) data movements. Cluster running at 290MHz and 1.2.}
    \label{fig:ae_results}
    \vspace{-4mm}
\end{figure}
The results are reported in Fig. \ref{fig:ae_results} in terms of execution latency and energy consumption. As expected, the \ac{TPE} delivers at least 10$\times$ speed-up with respect to a pure SW execution on all the layers of the \ac{AE} except for the latent space layers, where the performance improvement is reduced to 4-7 $\times$ due to lower arithmetic intensity of those layers. The matrix transposition performed with the tiny DataMover accelerator contributes to an additional 1-2 $\times$ of speed-up. Overall, combining the \ac{TPE} and the DataMover, the entire training epoch runs in 1.8 ms with an energy consumption of $345\,\mu J$, 13 $\times$ faster than the \textit{SW} execution of the \ac{AE} on the 8 RV-NN cores, with 14$\times$ lower energy consumption.

